Fast VEM Fluid Simulation

The intricate motion arising from fluid--boundary interactions is visually compelling, yet notoriously difficult and computationally expensive to simulate in the presence of complex boundaries. Accurately resolving boundary geometry requires body-fitted grids constructed via cut-cell methods, which often leads to poorly conditioned linear systems in the pressure projection stage and, consequently, prohibitive computational cost. We present FastVEM, an efficient boundary-conforming fluid simulation framework that enables high-fidelity flow--boundary interaction at substantially reduced cost. Computational efficiency is achieved through a coordinated, top-down design spanning numerical discretization, grid construction, and linear solvers. FastVEM adopts a Virtual Element Method (VEM) discretization to robustly enforce incompressibility and boundary conditions on irregular body-fitted grids, and employs a VEM polynomial-space Particle-in-Cell scheme for advection. Complementing this discretization, a convexity-preserving cut-cell strategy is introduced to construct simulation-friendly body-fitted grids. To accelerate pressure projection, we develop a Galerkin geometric multigrid solver featuring a diffusion-free prolongation operator that prevents coarse-level matrix densification, along with a nested, boundary-aware grid hierarchy that ensures well-posed placement of coarse-level degrees of freedom. Compared to prior cut-cell--based fluid simulators, FastVEM speeds up the computationally dominant pressure projection stage by up to 100x, while robustly handling even more challenging boundary geometries.

==> tables/conforming.tex <==
\begin{table}[]
\caption{rose}
\label{tab:conforming}
\centering
\rowcolors{1}{white}{gray!15}
\begin{tabular}{ccccc}
\hline
\textbf{Grid}          & \textbf{DOFs$^c$} & \textbf{DOFs$^{nc}$}& \textbf{Project$^c$/step} & \textbf{Project$^{nc}$/step} \\ \hline
16\textasciicircum{}3  &                     &     &                     &                     \\
32\textasciicircum{}3  &                     &    &                     &                    \\
64\textasciicircum{}3  &                     &     &                     &                    \\
128\textasciicircum{}3 &                     &     &                     &                   \\\hline
\end{tabular}
\end{table}
